Learning Node Representations from Noisy Graph Structures

Learning low-dimensional representations on graphs has proved to be effective in various downstream tasks. However, noises prevail in real-world networks, which compromise networks to a large extent in that edges in networks propagate noises through the whole network instead of only the node itself. While existing methods tend to focus on preserving structural properties, the robustness of the learned representations against noises is generally ignored. In this paper, we propose a novel framework to learn noise-free node representations and eliminate noises simultaneously. Since noises are often unknown on real graphs, we design two generators, namely a graph generator and a noise generator, to identify normal structures and noises in an unsupervised setting. On the one hand, the graph generator serves as a unified scheme to incorporate any useful graph prior knowledge to generate normal structures. We illustrate the generative process with community structures and power-law degree distributions as examples. On the other hand, the noise generator generates graph noises not only satisfying some fundamental properties but also in an adaptive way. Thus, real noises with arbitrary distributions can be handled successfully. Finally, in order to eliminate noises and obtain noise-free node representations, two generators need to be optimized jointly, and through maximum likelihood estimation, we equivalently convert the model into imposing different regularization constraints on the true graph and noises respectively. Our model is evaluated on both real-world and synthetic data. It outperforms other strong baselines for node classification and graph reconstruction tasks, demonstrating its ability to eliminate graph noises.

==> chaps/relatedwork.tex <==
\section{Related Work}

% \subsection{Tradition Network Embedding}
% 传统的网络表示学习方法，基于矩阵分解和神经网络，浅层网络和深层网络。这些方法都是假设网络是干净的，没有考虑网络在带噪声的情况下，增强网络表示向量的鲁棒性。
Tradition network embedding methods can be categorized into two types: SkipGram models like DeepWalk \cite{perozzi2014deepwalk} and LINE \cite{tang2015line}, and Graph neural networks like GCN \cite{kipf2016semi} and GraphSAGE \cite{hamilton2017inductive}. All these methods lack the ability to enhance the robustness of representations if graphs are corrupted.

% \subsection{Network Embedding with Noisy Data}
% 鲁棒网络表示学习
% 这些方法都是在向量空间中通学习表示向量，从而得到更稳定的表示结果，他们都不是专门针对网络结构中的噪声设计的，他们没有显示的定义，也没有利用先验知识，然而网络结构和网络噪声都是复杂的，这些方法并不能很好的过滤掉噪声。
Recently, some network embedding approaches to handle noisy data have been proposed. 
Most of them are mainly based on adversarial training, including AIDW \cite{dai2018adversarial}, ARGA \cite{pan2018adversarially}, NetRA \cite{yu2018learning}, GraphGAN \cite{wang2018graphgan} and AdvT \cite{dai2019adversarial}. For example, in AIDW and ARGA, representations are enforced to match a prior distribution via adversarial learning so that robust representations can be learned. 
Besides, there also have been some methods for enhancing the robustness of representations by handling the uncertainty of graph structure with the help of different techniques, including BGCN \cite{zhang2019bayesian} and RGCN \cite{zhu2019robust}. For example, BGCN is a Bayesian GCN framework that views the observed graph as a realization from parametric random graphs leading to better resilience to noises and attacks. 

Since all these methods work in vector space to obtain robust representations, none of them handle noises on graphs explicitly, and hence they cannot be extensible with prior knowledge of graph theories and noise properties. But our model, as the first one to learn noise-free representations in network space to the best of our knowledge, provides clear comprehensibility of real noises, so that different prior knowledge can be combined into. Therefore, the abilities of existing methods to learn robust representations are worse than our model, which will be proved in the experiments. 

